Brick Wall Quantum Circuits with Global Fermionic Symmetry

We study brick wall quantum circuits enjoying a global fermionic symmetry. The constituent 2-qubit gate, and its fermionic symmetry, derive from a 2-particle scattering matrix in integrable, supersymmetric quantum field theory in 1+1 dimensions. Our 2-qubit gate, as a function of three free parameters, is of so-called free fermionic or matchgate form, allowing us to derive the spectral structure of both the brick wall unitary $U_F$ and its, non-trivial, hamiltonian limit $H_{\gamma}$ in closed form. We find that the fermionic symmetry pins $H_{\gamma}$ to a surface of critical points, whereas breaking that symmetry leads to non-trivial topological phases. We briefly explore quench dynamics for this class of circuits.

==> answer_referees.tex <==
\section{Answer to the referees}

We thank the referees for their constructive criticisms and the many suggestions to improve our manuscript. In the revised version we followed the referees' suggestions and we modified or rewrote parts of the manuscript. The changes can be summarized as follows.

\begin{itemize}
    \item \textbf{major changes.} We expanded the introduction, adding more references to brick wall quantum circuits in different forms, clarifying notation issues and refining some parts to improve readability. In particular, we strengthened the motivation which brought us to investigate this class of quantum circuits, highlighting the underlying free fermionic structure and the global fermionic symmetry. We clearly formulated challenges and open questions for this class of circuits. We also pointed out the connection to QCAs, which corroborates our motivation to study regularized versions of QFTs endowed with supersymmetry. Furthermore, we followed the suggestions of the referees and we completely restructured section 5. We ran TEBD simulations of quench dynamics for large sizes and many layers of our brick wall unitary, focussing on the time evolution of single site magnetizations. We compared the findings with analytical reasoning based on the spectral structure that we uncovered, and showed that the equilibration of magnetizations can be captured by a GGE based on the free fermionic structure. We report a remarkable connection of our work to the recent work of Zadnik et al. We restructured the outlook in accordance with the changes made and added an appendix with some details of the quench dynamics for PBC.
    \item \textbf{minor changes.} We improved overall readability (especially in parts pointed out by the referees), corrected typos, expanded comments on graded tensor products and their relation to JW-transformations, expanded the explanation on the topological insulator part, explained further the role of global fermionic symmetry in the criticality of the Hamiltonian limits, clarified the difference between Hamiltonian limit and $\mathbf{U_F}$, explained unclear notations.
    
\end{itemize}

We are confident we touched upon all requested points and we remit to the referees for their judgement on the revised paper.

==> checklist.tex <==
%you can check items in the list by changing \item to \item[\done] 

\begin{itemize}
  \item Introduction
  \begin{todolist}
  \item clarify motivation
  \item make presentation more understandable for quantum info audience
  \item[\done] add references mentioned in report 2 (Proszen et al.,Chalker et al.)
  \item[\done] mention and add references to 8 vertex models 
  \item[\done] clarify Q notation of eqs. 1.1,1.4,1.5
  \item[\done] clarify that K in eq. 1.11 is 4x4 matrix. \textcolor{red}{It is not.}
  \item[\done] "In addition, under eq. 1.11, the Authors say K commutes with the sum of the supercharges, but the rapidity in Q changes, so is this still a commutation?"
  \item[\done] only one rapidity parameter in eq. 1.11 whereas in 1.5 there are 2. \textcolor{red}{Look at text above equation 1.7}
  \item  "I find the very last paragraph on page 4 cryptic (if it is supposed to convey relevant info, it should be rewritten)."
  \item[\done] clarify why S is better understood in fermionic language
  \item[\done] what does "a J-W transformation back to bosonic qubits in place" mean?
  \item[\done] " Under eq. 1.13 the Authors refer to qubits again. What are those qubits then; are these the degrees of freedom related via J-W transform to spins 1/2, operated upon by Pauli matrices (say those in eq. 1.4)?"
  \item[\done] "In eq. 2.3, rhs, the Authors probably meant $p(v_i) \rightarrow p(e_i)$"
  \item[\done] " The definition in eq. 2.4 is not clear. For example, what is the meaning of a “row (column) of a subspace”? "
  \item[\done] "What is the meaning of parity — with respect to which property of operators is it defined? For example, what is the parity of operator $\sigma_j^z$, where lower index is the site? What is instead the parity of a half-string $\prod_{i<j}\sigma^z_i$? Notice, that two half-strings ending at different positions commute. Aren’t half-strings supposed to be there in order to represent anticommuting operators?"
  \item[\done] provide simple examples of grading (e.g. JW transformation) to improve readability
  \end{todolist}


  
  \item Preliminaries
  \begin{todolist}
  \item[\done] in eq. 2.10 commutations miss RHS
  \item[\done]"The paragraph above eq. 2.11 is not very clearly written: the off-diagonal elements of what are referred to? If I understand correctly $S_{L,1}$ is special because the strings in the generalized J-W transformation do not cancel out and therefore a full parity operator remains? I think such additional explanations would be welcome: the reader should be aware, that the product in eq. 2.8 (for example), is an ordinary product of operators that are (mostly local), as in standard brickwork circuit. That is, apart from $S_{L,1}$."
  \item what is advantage of grading vs considering odd and even sectors separately, similarly to diagonalization of free models?
  \end{todolist}

  
  \item Hamiltonian limit
  \begin{todolist}
  \item[\done] eq. 3.1, is theta missing in the linear term in RHS?
  \item[\done] explain better that breaking of GFS does open a gap after eq. 3.7. refer to statement above eq. 3.6 to improve readability
  \item[\done] add references and context to BDI topological insulators (classic references are: Schnyder and Ludwig, Atland and Zirnbauer)
  \item[\done] after eq. 3.18 a brief comment on relevance of real vs imaginary delta
  \item[\done] redo sentence introducing  G and its motivation 
  \item[\done] explain that chirality is that of the hamiltonian limit, not of the full $U_F$
  \item[\done] deformed coefs in eq. 3.22 are introduced only in appendix B.1. Should refer to B.1 in main text
  \item[\done] express $Q's$ in term of fermionic annihilation and creation at end of sec. 2.4
  \item[\done] explain $|-\rangle$ notation in eq. 3.13
  \end{todolist}

  
  \item Spectral analysis
  \begin{todolist}
  \item[\done] explain $|-\rangle$ notation in eq. 4.9
  \end{todolist}

  
  \item Dynamics of entanglement
  \begin{todolist} 
  \item[\done] small size simulation considering f.f., improve size 
  \item PBC inverse Fourier transform for expectation vals of local operators and EE
  \item[\done] OBC TEBD simulations for $\sigma^{z}_j$
  \end{todolist}
\end{itemize}


